PolyCF: Towards the Optimal Spectral Graph Filters for Collaborative Filtering

Collaborative Filtering (CF) is a pivotal research area in recommender systems that capitalizes on collaborative similarities between users and items to provide personalized recommendations. With the remarkable achievements of node embedding-based Graph Neural Networks (GNNs), we explore the upper bounds of expressiveness inherent to embedding-based methodologies and tackle the challenges by reframing the CF task as a graph signal processing problem. To this end, we propose PolyCF, a flexible graph signal filter that leverages polynomial graph filters to process interaction signals. PolyCF exhibits the capability to capture spectral features across multiple eigenspaces through a series of Generalized Gram filters and is able to approximate the optimal polynomial response function for recovering missing interactions. A graph optimization objective and a pair-wise ranking objective are jointly used to optimize the parameters of the convolution kernel. Experiments on three widely adopted datasets demonstrate the superiority of PolyCF over current state-of-the-art CF methods. Moreover, comprehensive studies empirically validate each component's efficacy in the proposed PolyCF.

==> Tables/basis.tex <==
\begin{table*}[t]
\centering
\caption{Polynomial Basis used by \method{}.}
\label{tab:basis} 
\begin{tabular}{c |c|c|c}
\toprule %\hline
Basis & Definition of $P_k(\lambda)$ & Recurrent Form & Kernel Metric \\ 
% \midrule
\hline
Monomial & $P_k(\lambda)=\lambda^k$ & $P_{k+1}(\lambda)=P_{k}(\lambda)\lambda$ & N/A \\
Chebyshev-I & $\sum\limits_{k=0}^\infty P_k(\lambda)t^n=\frac{1-t\lambda}{1-2t\lambda+\lambda^2}$ & $P_{k+1}(\lambda)=2\lambda P_k(\lambda)-P_{k-1}(\lambda)$ & $\frac{1}{\sqrt{1-\lambda^2}}$ \\
Chebyshev-II & $\sum\limits_{k=0}^\infty P_k(\lambda)t^n=\frac{1}{1-2t\lambda+\lambda^2}$ & $P_{k+1}(\lambda)=2\lambda P_k(\lambda)-P_{k-1}(\lambda)$ & $\sqrt{1-\lambda^2}$ \\
Berstein & $P_k^{\nu}(\lambda)=\tbinom{k}{\nu}\lambda^\nu(1-\lambda)^{k-\nu}$ & $P_{k}^\nu(\lambda)=(1-\lambda)P_{k-1}^{\nu}(\lambda)+\lambda P_{k-1}^{\nu-1}(\lambda)$ & N/A \\
Laguerre & $P_k^{(\alpha)}(\lambda)=\sum\limits_{i=0}^k(-1)^i\tbinom{k+\alpha}{k-i}\frac{x^i}{i!}$ & $P_{k+1}(\lambda)=\frac{1}{k+1}((2k+1-\lambda)P_k(\lambda)-kP_{k-1}(\lambda))$ & $\lambda^\alpha e^{-\lambda}$ \\
Jacobi & $P_{k}^{\alpha,\beta}(\lambda)=\sum\limits_{s=0}^k\tbinom{k+\alpha}{s}\tbinom{k+\beta}{k-s}(\frac{\lambda-1}{2})^{k-s}(\frac{\lambda-1}{2})^{k+s}$ & $P_{k+1}^{\alpha,\beta}(\lambda)=(\lambda+1)P_k^{\alpha,\beta}(\lambda)-P_{k-1}^{\alpha,\beta}(\lambda)$ & $(1-\lambda)^\alpha(1-\lambda)^\beta$\\
Hermite & $P_k(\lambda)=(-1)^\lambda e^{\lambda^2}\frac{\mathrm{d}^k}{\mathrm{d}\lambda^k}e^{-\lambda^2}$ & $P_{k+1}(\lambda)=2\lambda P_k(\lambda)-2(n-1)P_{k-1}(\lambda)$ & $e^{-\lambda^2}$\\
\bottomrule % \hline
% \end{tabular}
\end{tabular}
\end{table*}
